Matryoshka attribution: Learning to attribute language model outputs to representations and weights

Attributing language model outputs to their internal computations is an open problem in interpretability. Existing methods, which use causal interventions, gradients, or learnable masks, either are infeasibly expensive or struggle to identify actual causally-important internal computations. We propose framing attribution as the problem of identifying nested subsets of internal components which minimise a downstream loss. To learn this task, we introduce Matryoshka Attribution (MAttr), a mask learning method that parametrises the mask with a simple differentiable sigmoid top-$k$ operator. We supervise training over all sparsities simultaneously by randomising $k$ over training, resulting in a learned ordering of components by attribution score. MAttr achieves number 1 on the official leaderboard of the Mechanistic Interpretability Benchmark (Mueller et al., 2025); our method identifies sparse and task-transferrable circuits across varying circuit bases. As a practical application, we show that MAttr can be trained with reinforcement learning to identify weight changes responsible for downstream behaviours in LLM finetuning. We train MAttr on refusal judge scores and find that restoring $1\%$ of Llama 3.1 8B Instruct's weights to their base model state is sufficient to remove refusals while maintaining capabilities. We view MAttr as a successful formulation of interpretability into a learnable objective that we can tackle with gradient descent, and encourage future work along these lines.

==> tabs/sva_top_neurons.tex <==
% Requires \usepackage{booktabs,longtable,colortbl,hyperref}; \input at top level (NOT inside a table float).
\definecolor{recur0}{HTML}{FBB4AE}
\definecolor{recur1}{HTML}{B3CDE3}
\definecolor{recur2}{HTML}{CCEBC5}
\definecolor{recur3}{HTML}{DECBE4}
\definecolor{recur4}{HTML}{FED9A6}
\definecolor{recur5}{HTML}{8DD3C7}
\definecolor{recur6}{HTML}{E8DE6B}
{\scriptsize
\setlength{\tabcolsep}{3pt}
\setlength{\fboxsep}{1pt}
\renewcommand{\arraystretch}{1.15}
\begin{longtable}{@{}l *{7}{>{\raggedright\arraybackslash}p{0.125\textwidth}}@{}}
\toprule
& \textbf{IG} & \textbf{I$\times$G} & \textbf{Node Pruning} & \textbf{DBM} & \textbf{\ourmethod{}} & \textbf{\ourmethod{} $+$ unif $k$} & \textbf{\ourmethod{} $+$ SGD} \\
\midrule
\endfirsthead
\toprule
& \textbf{IG} & \textbf{I$\times$G} & \textbf{Node Pruning} & \textbf{DBM} & \textbf{\ourmethod{}} & \textbf{\ourmethod{} $+$ unif $k$} & \textbf{\ourmethod{} $+$ SGD} \\
\midrule
\endhead
\bottomrule
\multicolumn{8}{@{}p{0.97\textwidth}@{}}{\scriptsize Recurring in $\geq$10 of the 56 cells:~\colorbox{recur0}{$\ell$1.n6746}~$\times$13\quad \colorbox{recur1}{$\ell$0.n1015}~$\times$12\quad \colorbox{recur2}{$\ell$2.n1857}~$\times$11\quad \colorbox{recur3}{$\ell$0.n6144}~$\times$10\quad \colorbox{recur4}{$\ell$18.n1712}~$\times$10\quad \colorbox{recur5}{$\ell$26.n2322}~$\times$10\quad \colorbox{recur6}{$\ell$30.n11158}~$\times$10} \\
\multicolumn{8}{@{}p{0.97\textwidth}@{}}{\scriptsize Marks apply to the 4 arithmetic blocks only, against each task's own published set:~$^{\star}$~one of the 15--28 layer-18 MLP neurons \citet{feucht2026arithmetic} localise that task's cyclic arithmetic to (13 occurrences here)} \\
\endlastfoot
\multicolumn{8}{@{}l}{\textsc{\textbf{Logit difference} loss}} \\*[3pt]
\multicolumn{8}{@{}l}{\textbf{Simple}} \\*[2pt]
1. & \href{https://neurons.transluce.org/0/1015/+}{\colorbox{recur1}{$\ell$0.n1015}.p2} & \href{https://neurons.transluce.org/30/11158/+}{\colorbox{recur6}{$\ell$30.n11158}.p2} & \href{https://neurons.transluce.org/31/14249/+}{$\ell$31.n14249.p2} & \href{https://neurons.transluce.org/31/10088/+}{$\ell$31.n10088.p2} & \href{https://neurons.transluce.org/0/1015/+}{\colorbox{recur1}{$\ell$0.n1015}.p2} & \href{https://neurons.transluce.org/31/10088/+}{$\ell$31.n10088.p2} & \href{https://neurons.transluce.org/0/1015/+}{\colorbox{recur1}{$\ell$0.n1015}.p2} \\
\rowcolor[HTML]{F7F7F7}2. & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p2} & \href{https://neurons.transluce.org/31/11075/+}{$\ell$31.n11075.p2} & \href{https://neurons.transluce.org/31/13161/+}{$\ell$31.n13161.p2} & \href{https://neurons.transluce.org/29/8432/+}{$\ell$29.n8432.p2} & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p2} & \href{https://neurons.transluce.org/22/4703/+}{$\ell$22.n4703.p2} & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p2} \\
3. & \href{https://neurons.transluce.org/3/11818/+}{$\ell$3.n11818.p2} & \href{https://neurons.transluce.org/19/12056/+}{$\ell$19.n12056.p2} & \href{https://neurons.transluce.org/31/5357/+}{$\ell$31.n5357.p2} & \href{https://neurons.transluce.org/16/2319/+}{$\ell$16.n2319.p2} & \href{https://neurons.transluce.org/17/13649/+}{$\ell$17.n13649.p2} & \href{https://neurons.transluce.org/4/6753/+}{$\ell$4.n6753.p2} & \href{https://neurons.transluce.org/3/11818/+}{$\ell$3.n11818.p2} \\
\rowcolor[HTML]{F7F7F7}4. & \href{https://neurons.transluce.org/0/6144/+}{\colorbox{recur3}{$\ell$0.n6144}.p2} & \href{https://neurons.transluce.org/31/5287/+}{$\ell$31.n5287.p2} & \href{https://neurons.transluce.org/31/2139/+}{$\ell$31.n2139.p2} & \href{https://neurons.transluce.org/31/11059/+}{$\ell$31.n11059.p2} & \href{https://neurons.transluce.org/3/11818/+}{$\ell$3.n11818.p2} & \href{https://neurons.transluce.org/2/1857/+}{\colorbox{recur2}{$\ell$2.n1857}.p2} & \href{https://neurons.transluce.org/2/1857/+}{\colorbox{recur2}{$\ell$2.n1857}.p2} \\
5. & \href{https://neurons.transluce.org/30/11158/+}{\colorbox{recur6}{$\ell$30.n11158}.p2} & \href{https://neurons.transluce.org/31/10088/+}{$\ell$31.n10088.p2} & \href{https://neurons.transluce.org/31/7969/+}{$\ell$31.n7969.p2} & \href{https://neurons.transluce.org/18/3902/+}{$\ell$18.n3902.p2} & \href{https://neurons.transluce.org/2/1857/+}{\colorbox{recur2}{$\ell$2.n1857}.p2} & \href{https://neurons.transluce.org/31/11075/+}{$\ell$31.n11075.p2} & \href{https://neurons.transluce.org/17/13649/+}{$\ell$17.n13649.p2} \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Noun PP}} \\*[2pt]
1. & \href{https://neurons.transluce.org/0/1015/+}{\colorbox{recur1}{$\ell$0.n1015}.p2} & \href{https://neurons.transluce.org/30/11158/+}{\colorbox{recur6}{$\ell$30.n11158}.p5} & \href{https://neurons.transluce.org/31/6636/+}{$\ell$31.n6636.p5} & \href{https://neurons.transluce.org/14/7990/+}{$\ell$14.n7990.p4} & \href{https://neurons.transluce.org/0/1015/+}{\colorbox{recur1}{$\ell$0.n1015}.p2} & \href{https://neurons.transluce.org/31/10088/+}{$\ell$31.n10088.p5} & \href{https://neurons.transluce.org/0/1015/+}{\colorbox{recur1}{$\ell$0.n1015}.p2} \\
\rowcolor[HTML]{F7F7F7}2. & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p2} & \href{https://neurons.transluce.org/29/10537/+}{$\ell$29.n10537.p5} & \href{https://neurons.transluce.org/31/9242/+}{$\ell$31.n9242.p5} & \href{https://neurons.transluce.org/8/4032/+}{$\ell$8.n4032.p4} & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p2} & \href{https://neurons.transluce.org/29/13065/+}{$\ell$29.n13065.p5} & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p2} \\
3. & \href{https://neurons.transluce.org/0/6144/+}{\colorbox{recur3}{$\ell$0.n6144}.p2} & \href{https://neurons.transluce.org/31/11075/+}{$\ell$31.n11075.p5} & \href{https://neurons.transluce.org/31/6685/+}{$\ell$31.n6685.p5} & \href{https://neurons.transluce.org/20/14243/+}{$\ell$20.n14243.p5} & \href{https://neurons.transluce.org/2/1857/+}{\colorbox{recur2}{$\ell$2.n1857}.p2} & \href{https://neurons.transluce.org/30/11158/+}{\colorbox{recur6}{$\ell$30.n11158}.p5} & \href{https://neurons.transluce.org/2/1857/+}{\colorbox{recur2}{$\ell$2.n1857}.p2} \\
\rowcolor[HTML]{F7F7F7}4. & \href{https://neurons.transluce.org/3/11818/+}{$\ell$3.n11818.p2} & \href{https://neurons.transluce.org/31/5287/+}{$\ell$31.n5287.p5} & \href{https://neurons.transluce.org/20/2840/+}{$\ell$20.n2840.p4} & \href{https://neurons.transluce.org/31/4501/+}{$\ell$31.n4501.p5} & \href{https://neurons.transluce.org/0/6144/+}{\colorbox{recur3}{$\ell$0.n6144}.p2} & \href{https://neurons.transluce.org/4/6753/+}{$\ell$4.n6753.p2} & \href{https://neurons.transluce.org/0/6144/+}{\colorbox{recur3}{$\ell$0.n6144}.p2} \\
5. & \href{https://neurons.transluce.org/30/11158/+}{\colorbox{recur6}{$\ell$30.n11158}.p5} & \href{https://neurons.transluce.org/30/13476/+}{$\ell$30.n13476.p5} & \href{https://neurons.transluce.org/31/3382/+}{$\ell$31.n3382.p5} & \href{https://neurons.transluce.org/27/708/+}{$\ell$27.n708.p5} & \href{https://neurons.transluce.org/4/6753/+}{$\ell$4.n6753.p2} & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p2} & \href{https://neurons.transluce.org/3/11818/+}{$\ell$3.n11818.p2} \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{RC}} \\*[2pt]
1. & \href{https://neurons.transluce.org/0/1015/+}{\colorbox{recur1}{$\ell$0.n1015}.p2} & \href{https://neurons.transluce.org/30/11158/+}{\colorbox{recur6}{$\ell$30.n11158}.p6} & \href{https://neurons.transluce.org/31/12120/+}{$\ell$31.n12120.p6} & \href{https://neurons.transluce.org/30/1110/+}{$\ell$30.n1110.p6} & \href{https://neurons.transluce.org/0/1015/+}{\colorbox{recur1}{$\ell$0.n1015}.p2} & \href{https://neurons.transluce.org/31/10088/+}{$\ell$31.n10088.p6} & \href{https://neurons.transluce.org/0/1015/+}{\colorbox{recur1}{$\ell$0.n1015}.p2} \\
\rowcolor[HTML]{F7F7F7}2. & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p2} & \href{https://neurons.transluce.org/29/10537/+}{$\ell$29.n10537.p6} & \href{https://neurons.transluce.org/30/4984/+}{$\ell$30.n4984.p2} & \href{https://neurons.transluce.org/15/1574/+}{$\ell$15.n1574.p4} & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p2} & \href{https://neurons.transluce.org/29/13065/+}{$\ell$29.n13065.p6} & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p2} \\
3. & \href{https://neurons.transluce.org/30/11158/+}{\colorbox{recur6}{$\ell$30.n11158}.p6} & \href{https://neurons.transluce.org/20/7715/+}{$\ell$20.n7715.p6} & \href{https://neurons.transluce.org/29/10654/+}{$\ell$29.n10654.p3} & \href{https://neurons.transluce.org/30/7745/+}{$\ell$30.n7745.p6} & \href{https://neurons.transluce.org/2/1857/+}{\colorbox{recur2}{$\ell$2.n1857}.p2} & \href{https://neurons.transluce.org/30/11158/+}{\colorbox{recur6}{$\ell$30.n11158}.p6} & \href{https://neurons.transluce.org/2/1857/+}{\colorbox{recur2}{$\ell$2.n1857}.p2} \\
\rowcolor[HTML]{F7F7F7}4. & \href{https://neurons.transluce.org/0/6144/+}{\colorbox{recur3}{$\ell$0.n6144}.p2} & \href{https://neurons.transluce.org/31/11075/+}{$\ell$31.n11075.p6} & \href{https://neurons.transluce.org/30/9818/+}{$\ell$30.n9818.p4} & \href{https://neurons.transluce.org/22/8478/+}{$\ell$22.n8478.p6} & \href{https://neurons.transluce.org/18/13748/+}{$\ell$18.n13748.p6} & \href{https://neurons.transluce.org/29/10537/+}{$\ell$29.n10537.p6} & \href{https://neurons.transluce.org/18/13748/+}{$\ell$18.n13748.p6} \\
5. & \href{https://neurons.transluce.org/2/1857/+}{\colorbox{recur2}{$\ell$2.n1857}.p2} & \href{https://neurons.transluce.org/19/12056/+}{$\ell$19.n12056.p6} & \href{https://neurons.transluce.org/31/7964/+}{$\ell$31.n7964.p6} & \href{https://neurons.transluce.org/31/5540/+}{$\ell$31.n5540.p6} & \href{https://neurons.transluce.org/0/6144/+}{\colorbox{recur3}{$\ell$0.n6144}.p2} & \href{https://neurons.transluce.org/31/11075/+}{$\ell$31.n11075.p6} & \href{https://neurons.transluce.org/0/6144/+}{\colorbox{recur3}{$\ell$0.n6144}.p2} \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Within RC}} \\*[2pt]
1. & \href{https://neurons.transluce.org/0/1015/+}{\colorbox{recur1}{$\ell$0.n1015}.p5} & \href{https://neurons.transluce.org/30/11158/+}{\colorbox{recur6}{$\ell$30.n11158}.p5} & \href{https://neurons.transluce.org/31/6685/+}{$\ell$31.n6685.p5} & \href{https://neurons.transluce.org/31/4112/+}{$\ell$31.n4112.p5} & \href{https://neurons.transluce.org/0/1015/+}{\colorbox{recur1}{$\ell$0.n1015}.p5} & \href{https://neurons.transluce.org/31/10088/+}{$\ell$31.n10088.p5} & \href{https://neurons.transluce.org/0/1015/+}{\colorbox{recur1}{$\ell$0.n1015}.p5} \\
\rowcolor[HTML]{F7F7F7}2. & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p5} & \href{https://neurons.transluce.org/31/11075/+}{$\ell$31.n11075.p5} & \href{https://neurons.transluce.org/31/13222/+}{$\ell$31.n13222.p5} & \href{https://neurons.transluce.org/12/2243/+}{$\ell$12.n2243.p5} & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p5} & \href{https://neurons.transluce.org/29/13065/+}{$\ell$29.n13065.p5} & \href{https://neurons.transluce.org/1/6746/+}{\colorbox{recur0}{$\ell$1.n6746}.p5} \\
3. & \href{https://neurons.transluce.org/0/6144/+}{\colorbox{recur3}{$\ell$0.n6144}.p5} & \href{https://neurons.transluce.org/19/12056/+}{$\ell$19.n12056.p5} & \href{https://neurons.transluce.org/31/9242/+}{$\ell$31.n9242.p5} & \href{https://neurons.transluce.org/19/464/+}{$\ell$19.n464.p5} & \href{https://neurons.transluce.org/2/1857/+}{\colorbox{recur2}{$\ell$2.n1857}.p5} & \href{https://neurons.transluce.org/4/6753/+}{$\ell$4.n6753.p5} & \href{https://neurons.transluce.org/2/1857/+}{\colorbox{recur2}{$\ell$2.n1857}.p5} \\
\rowcolor[HTML]{F7F7F7}4. & \href{https://neurons.transluce.org/3/11818/+}{$\ell$3.n11818.p5} & \href{https://neurons.transluce.org/25/529/+}{$\ell$25.n529.p5} & \href{https://neurons.transluce.org/31/5503/+}{$\ell$31.n5503.p5} & \href{https://neurons.transluce.org/30/1969/+}{$\ell$30.n1969.p5} & \href{https://neurons.transluce.org/0/6144/+}{\colorbox{recur3}{$\ell$0.n6144}.p5} & \href{https://neurons.transluce.org/30/11158/+}{\colorbox{recur6}{$\ell$30.n11158}.p5} & \href{https://neurons.transluce.org/0/6144/+}{\colorbox{recur3}{$\ell$0.n6144}.p5} \\
5. & \href{https://neurons.transluce.org/2/1857/+}{\colorbox{recur2}{$\ell$2.n1857}.p5} & \href{https://neurons.transluce.org/26/11122/+}{$\ell$26.n11122.p5} & \href{https://neurons.transluce.org/31/12128/+}{$\ell$31.n12128.p5} & \href{https://neurons.transluce.org/31/5831/+}{$\ell$31.n5831.p5} & \href{https://neurons.transluce.org/4/6753/+}{$\ell$4.n6753.p5} & \href{https://neurons.transluce.org/22/4703/+}{$\ell$22.n4703.p5} & \href{https://neurons.transluce.org/4/6753/+}{$\ell$4.n6753.p5} \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Addition}} \\*[2pt]
1. & \href{https://neurons.transluce.org/15/7446/+}{$\ell$15.n7446.p4} & \href{https://neurons.transluce.org/27/7993/+}{$\ell$27.n7993.p4} & \href{https://neurons.transluce.org/31/11015/+}{$\ell$31.n11015.p4} & \href{https://neurons.transluce.org/31/3066/+}{$\ell$31.n3066.p4} & \href{https://neurons.transluce.org/18/1712/+}{\colorbox{recur4}{$\ell$18.n1712}.p4$^{\star}$} & \href{https://neurons.transluce.org/18/1712/+}{\colorbox{recur4}{$\ell$18.n1712}.p4$^{\star}$} & \href{https://neurons.transluce.org/18/1712/+}{\colorbox{recur4}{$\ell$18.n1712}.p4$^{\star}$} \\
\rowcolor[HTML]{F7F7F7}2. & \href{https://neurons.transluce.org/15/130/+}{$\ell$15.n130.p4} & \href{https://neurons.transluce.org/24/12439/+}{$\ell$24.n12439.p4} & \href{https://neurons.transluce.org/27/3082/+}{$\ell$27.n3082.p3} & \href{https://neurons.transluce.org/23/510/+}{$\ell$23.n510.p4} & \href{https://neurons.transluce.org/21/9178/+}{$\ell$21.n9178.p4} & \href{https://neurons.transluce.org/0/14115/+}{$\ell$0.n14115.p3} & \href{https://neurons.transluce.org/21/9178/+}{$\ell$21.n9178.p4} \\
3. & \href{https://neurons.transluce.org/22/13088/+}{$\ell$22.n13088.p4} & \href{https://neurons.transluce.org/23/510/+}{$\ell$23.n510.p4} & \href{https://neurons.transluce.org/31/2398/+}{$\ell$31.n2398.p4} & \href{https://neurons.transluce.org/18/3134/+}{$\ell$18.n3134.p4} & \href{https://neurons.transluce.org/26/2322/+}{\colorbox{recur5}{$\ell$26.n2322}.p4} & \href{https://neurons.transluce.org/15/12769/+}{$\ell$15.n12769.p4} & \href{https://neurons.transluce.org/15/13664/+}{$\ell$15.n13664.p4} \\
\rowcolor[HTML]{F7F7F7}4. & \href{https://neurons.transluce.org/27/7993/+}{$\ell$27.n7993.p4} & \href{https://neurons.transluce.org/22/13088/+}{$\ell$22.n13088.p4} & \href{https://neurons.transluce.org/29/6756/+}{$\ell$29.n6756.p2} & \href{https://neurons.transluce.org/11/9066/+}{$\ell$11.n9066.p4} & \href{https://neurons.transluce.org/15/13664/+}{$\ell$15.n13664.p4} & \href{https://neurons.transluce.org/15/130/+}{$\ell$15.n130.p4} & \href{https://neurons.transluce.org/20/9747/+}{$\ell$20.n9747.p4} \\
5. & \href{https://neurons.transluce.org/20/11837/+}{$\ell$20.n11837.p4} & \href{https://neurons.transluce.org/25/6283/+}{$\ell$25.n6283.p4} & \href{https://neurons.transluce.org/31/9576/+}{$\ell$31.n9576.p4} & \href{https://neurons.transluce.org/28/13336/+}{$\ell$28.n13336.p4} & \href{https://neurons.transluce.org/20/9747/+}{$\ell$20.n9747.p4} & \href{https://neurons.transluce.org/0/5095/+}{$\ell$0.n5095.p3} & \href{https://neurons.transluce.org/4/3465/+}{$\ell$4.n3465.p3} \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Months}} \\*[2pt]
1. & \href{https://neurons.transluce.org/26/2322/+}{\colorbox{recur5}{$\ell$26.n2322}.p12} & \href{https://neurons.transluce.org/22/3927/+}{$\ell$22.n3927.p12} & \href{https://neurons.transluce.org/25/14202/+}{$\ell$25.n14202.p2} & \href{https://neurons.transluce.org/3/10410/+}{$\ell$3.n10410.p5} & \href{https://neurons.transluce.org/18/1712/+}{\colorbox{recur4}{$\ell$18.n1712}.p12$^{\star}$} & \href{https://neurons.transluce.org/18/1712/+}{\colorbox{recur4}{$\ell$18.n1712}.p12$^{\star}$} & \href{https://neurons.transluce.org/18/1712/+}{\colorbox{recur4}{$\ell$18.n1712}.p12$^{\star}$} \\
\rowcolor[HTML]{F7F7F7}2. & \href{https://neurons.transluce.org/22/3927/+}{$\ell$22.n3927.p12} & \href{https://neurons.transluce.org/26/2322/+}{\colorbox{recur5}{$\ell$26.n2322}.p12} & \href{https://neurons.transluce.org/30/13584/+}{$\ell$30.n13584.p8} & \href{https://neurons.transluce.org/24/1102/+}{$\ell$24.n1102.p11} & \href{https://neurons.transluce.org/26/2322/+}{\colorbox{recur5}{$\ell$26.n2322}.p12} & \href{https://neurons.transluce.org/26/2322/+}{\colorbox{recur5}{$\ell$26.n2322}.p12} & \href{https://neurons.transluce.org/26/2322/+}{\colorbox{recur5}{$\ell$26.n2322}.p12} \\
3. & \href{https://neurons.transluce.org/18/1712/+}{\colorbox{recur4}{$\ell$18.n1712}.p12$^{\star}$} & \href{https://neurons.transluce.org/23/9030/+}{$\ell$23.n9030.p12} & \href{https://neurons.transluce.org/28/9388/+}{$\ell$28.n9388.p3} & \href{https://neurons.transluce.org/9/7457/+}{$\ell$9.n7457.p11} & \href{https://neurons.transluce.org/17/13232/+}{$\ell$17.n13232.p12} & \href{https://neurons.transluce.org/18/8409/+}{$\ell$18.n8409.p12$^{\star}$} & \href{https://neurons.transluce.org/15/13664/+}{$\ell$15.n13664.p12} \\
\rowcolor[HTML]{F7F7F7}4. & \href{https://neurons.transluce.org/18/12154/+}{$\ell$18.n12154.p12$^{\star}$} & \href{https://neurons.transluce.org/29/10808/+}{$\ell$29.n10808.p12} & \href{https://neurons.transluce.org/20/10839/+}{$\ell$20.n10839.p2} & \href{https://neurons.transluce.org/4/9258/+}{$\ell$4.n9258.p5} & \href{https://neurons.transluce.org/15/13664/+}{$\ell$15.n13664.p12} & \href{https://neurons.transluce.org/3/11799/+}{$\ell$3.n11799.p9} & \href{https://neurons.transluce.org/21/9178/+}{$\ell$21.n9178.p12} \\
5. & \href{https://neurons.transluce.org/25/3983/+}{$\ell$25.n3983.p12} & \href{https://neurons.transluce.org/25/3983/+}{$\ell$25.n3983.p12} & \href{https://neurons.transluce.org/21/4319/+}{$\ell$21.n4319.p3} & \href{https://neurons.transluce.org/6/7137/+}{$\ell$6.n7137.p3} & \href{https://neurons.transluce.org/21/9178/+}{$\ell$21.n9178.p12} & \href{https://neurons.transluce.org/22/9758/+}{$\ell$22.n9758.p12} & \href{https://neurons.transluce.org/17/13232/+}{$\ell$17.n13232.p12} \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Weekdays}} \\*[2pt]
1. & \href{https://neurons.transluce.org/21/12716/+}{$\ell$21.n12716.p12} & \href{https://neurons.transluce.org/21/12716/+}{$\ell$21.n12716.p12} & \href{https://neurons.transluce.org/24/5015/+}{$\ell$24.n5015.p3} & \href{https://neurons.transluce.org/14/10878/+}{$\ell$14.n10878.p10} & \href{https://neurons.transluce.org/22/6468/+}{$\ell$22.n6468.p12} & \href{https://neurons.transluce.org/25/1092/+}{$\ell$25.n1092.p12} & \href{https://neurons.transluce.org/20/3179/+}{$\ell$20.n3179.p12} \\
\rowcolor[HTML]{F7F7F7}2. & \href{https://neurons.transluce.org/20/3179/+}{$\ell$20.n3179.p12} & \href{https://neurons.transluce.org/20/3179/+}{$\ell$20.n3179.p12} & \href{https://neurons.transluce.org/27/3449/+}{$\ell$27.n3449.p3} & \href{https://neurons.transluce.org/29/12010/+}{$\ell$29.n12010.p12} & \href{https://neurons.transluce.org/20/3179/+}{$\ell$20.n3179.p12} & \href{https://neurons.transluce.org/23/5868/+}{$\ell$23.n5868.p12} & \href{https://neurons.transluce.org/23/5868/+}{$\ell$23.n5868.p12} \\
3. & \href{https://neurons.transluce.org/23/5868/+}{$\ell$23.n5868.p12} & \href{https://neurons.transluce.org/27/13859/+}{$\ell$27.n13859.p12} & \href{https://neurons.transluce.org/29/5193/+}{$\ell$29.n5193.p3} & \href{https://neurons.transluce.org/12/14160/+}{$\ell$12.n14160.p10} & \href{https://neurons.transluce.org/23/5868/+}{$\ell$23.n5868.p12} & \href{https://neurons.transluce.org/21/12716/+}{$\ell$21.n12716.p12} & \href{https://neurons.transluce.org/19/4639/+}{$\ell$19.n4639.p12} \\
\rowcolor[HTML]{F7F7F7}4. & \href{https://neurons.transluce.org/27/13859/+}{$\ell$27.n13859.p12} & \href{https://neurons.transluce.org/23/5868/+}{$\ell$23.n5868.p12} & \href{https://neurons.transluce.org/30/9614/+}{$\ell$30.n9614.p3} & \href{https://neurons.transluce.org/31/4876/+}{$\ell$31.n4876.p12} & \href{https://neurons.transluce.org/25/1092/+}{$\ell$25.n1092.p12} & \href{https://neurons.transluce.org/22/12637/+}{$\ell$22.n12637.p12} & \href{https://neurons.transluce.org/22/6468/+}{$\ell$22.n6468.p12} \\
5. & \href{https://neurons.transluce.org/15/9205/+}{$\ell$15.n9205.p12} & \href{https://neurons.transluce.org/22/6468/+}{$\ell$22.n6468.p12} & \href{https://neurons.transluce.org/29/1954/+}{$\ell$29.n1954.p2} & \href{https://neurons.transluce.org/13/776/+}{$\ell$13.n776.p10} & \href{https://neurons.transluce.org/18/11029/+}{$\ell$18.n11029.p12$^{\star}$} & \href{https://neurons.transluce.org/20/3179/+}{$\ell$20.n3179.p12} & \href{https://neurons.transluce.org/27/13859/+}{$\ell$27.n13859.p12} \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Hours}} \\*[2pt]
1. & \href{https://neurons.transluce.org/26/2322/+}{\colorbox{recur5}{$\ell$26.n2322}.p37} & \href{https://neurons.transluce.org/26/2322/+}{\colorbox{recur5}{$\ell$26.n2322}.p37} & \href{https://neurons.transluce.org/30/182/+}{$\ell$30.n182.p11} & \href{https://neurons.transluce.org/5/14152/+}{$\ell$5.n14152.p7} & \href{https://neurons.transluce.org/26/2322/+}{\colorbox{recur5}{$\ell$26.n2322}.p37} & \href{https://neurons.transluce.org/31/12785/+}{$\ell$31.n12785.p37} & \href{https://neurons.transluce.org/26/2322/+}{\colorbox{recur5}{$\ell$26.n2322}.p37} \\
\rowcolor[HTML]{F7F7F7}2. & \href{https://neurons.transluce.org/18/1712/+}{\colorbox{recur4}{$\ell$18.n1712}.p37$^{\star}$} & \href{https://neurons.transluce.org/22/13922/+}{$\ell$22.n13922.p37} & \href{https://neurons.transluce.org/30/5175/+}{$\ell$30.n5175.p11} & \href{https://neurons.transluce.org/9/13728/+}{$\ell$9.n13728.p10} & \href{https://neurons.transluce.org/17/13232/+}{$\ell$17.n13232.p37} & \href{https://neurons.transluce.org/24/5945/+}{$\ell$24.n5945.p37} & \href{https://neurons.transluce.org/17/13232/+}{$\ell$17.n13232.p37} \\
3. & \href{https://neurons.transluce.org/19/489/+}{$\ell$19.n489.p37} & \href{https://neurons.transluce.org/31/5392/+}{$\ell$31.n5392.p37} & \href{https://neurons.transluce.org/23/4845/+}{$\ell$23.n4845.p34} & \href{https://neurons.transluce.org/8/11592/+}{$\ell$8.n11592.p7} & \href{https://neurons.transluce.org/18/1712/+}{\colorbox{recur4}{$\ell$18.n1712}.p37$^{\star}$} & \href{https://neurons.transluce.org/22/13922/+}{$\ell$22.n13922.p37} & \href{https://neurons.transluce.org/18/1712/+}{\colorbox{recur4}{$\ell$18.n1712}.p37$^{\star}$} \\
\rowcolor[HTML]{F7F7F7}4. & \href{https://neurons.transluce.org/15/13664/+}{$\ell$15.n13664.p37} & \href{https://neurons.transluce.org/28/67/+}{$\ell$28.n67.p37} & \href{https://neurons.transluce.org/27/9397/+}{$\ell$27.n9397.p16} & \href{https://neurons.transluce.org/4/5014/+}{$\ell$4.n5014.p7} & \href{https://neurons.transluce.org/21/9178/+}{$\ell$21.n9178.p37} & \href{https://neurons.transluce.org/15/7446/+}{$\ell$15.n7446.p37} & \href{https://neurons.transluce.org/21/9178/+}{$\ell$21.n9178.p37} \\
5. & \href{https://neurons.transluce.org/22/13922/+}{$\ell$22.n13922.p37} & \href{https://neurons.transluce.org/30/6129/+}{$\ell$30.n6129.p37} & \href{https://neurons.transluce.org/30/14310/+}{$\ell$30.n14310.p10} & \href{https://neurons.transluce.org/4/2435/+}{$\ell$4.n2435.p7} & \href{https://neurons.transluce.org/19/9981/+}{$\ell$19.n9981.p37} & \href{https://neurons.transluce.org/28/774/+}{$\ell$28.n774.p37} & \href{https://neurons.transluce.org/19/9981/+}{$\ell$19.n9981.p37} \\
\end{longtable}
}

